Can LLMs Reason Over Non-Text Modalities in a Training-Free Manner? A Case Study with In-Context Representation Learning

The remarkable performance of Large Language Models (LLMs) can be enhanced with test-time computation, which relies on external tools and even other deep learning models. However, existing approaches for integrating non-text modality representations into LLMs typically require additional costly supervised training, restricting on-the-fly adaptation to new domains and modalities. In this work, we explore the feasibility of integrating representations from non-text foundational models (FMs) into text-based LLMs in a training-free manner. We propose In-Context Representation Learning (ICRL) as a proof-of-concept to allow LLMs to adaptively utilize non-text modality representations with few-shot learning. Unlike traditional in-context learning, which incorporates text-label pairs, ICRL replaces text inputs with FM representations, enabling the LLM to perform multi-modal inference without fine-tuning. We evaluate ICRL on a suite of tasks in the molecular domain, investigating three core research questions: (i) how to map FM representations into LLMs in a training-free manner, (ii) what factors influence ICRL performance, and (iii) what mechanisms underlie the effectiveness of ICRL. To the best of our knowledge, ICRL is the first training-free framework for integrating non-text modality representations into text-based LLMs, presenting a promising direction for adaptable, multi-modal generalization.

==> Tables/project_with_act.tex <==
\begin{table*}[!ht]
\caption{
Performance comparison on the ESOL dataset. 
\textbf{Bold} = best value (highest for \textit{Pearson}/\textit{Spearman}, lowest for \textit{RMSE}); 
\underline{Underline} = second-best.
}
\label{tab:esol_comparison_pivot}
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule
 & 
\multicolumn{2}{c}{\textbf{Ran-Pro (Act)}} & 
\multicolumn{2}{c}{\textbf{Matrix OT}} & 
\multicolumn{2}{c}{\textbf{OT-PCA (Act)}} & 
\multicolumn{2}{c}{\textbf{SF Projector}} & 
\multicolumn{2}{c}{\textbf{OT-Embed (Act)}}
\\

\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}

\textbf{Metric}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
\\
\midrule

%-----------------------------
% PEARSON
%-----------------------------
\textbf{Pearson} & 
0.193  & 0.140 &   % Ran-Pro(Act)
0.193  & 0.140 &   % Matrix OT
0.282  & 0.254 &   % OT-PCA (Act)
0.171  & 0.127 &   % SF Projector
0.264  & 0.269 &   % OT-Embed (Act)
\\

%-----------------------------
% SPEARMAN
%-----------------------------
\textbf{Spearman} &
0.175  & 0.145 &   % Ran-Pro(Act)
0.175  & 0.145 &   % Matrix OT
0.285  & 0.239 &   % OT-PCA (Act)
0.150  & 0.120 &   % SF Projector
0.269  & 0.274 &   % OT-Embed (Act)
\\

%-----------------------------
% RMSE
%-----------------------------
\textbf{RMSE} &
1.279 & 1.284 &  % Ran-Pro(Act)
1.279 & 1.284 &  % Matrix OT
1.225 & 1.216 &  % OT-PCA (Act)
1.644 & 1.408 &  % SF Projector
1.262 & 1.244 &  % OT-Embed (Act)
\\

\bottomrule
\end{tabular}
}
\end{table*}



\begin{table*}[!ht]

\caption{
\textbf{ICL Methods} on ESOL dataset. \\
\textbf{Bold} = best value (highest for \textit{Pearson}/\textit{Spearman}, lowest for \textit{RMSE}); 
\underline{Underline} = second-best.
}
\label{tab:esol_comparison_ICL_matched}
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
 & 
\multicolumn{2}{c}{\textbf{Ran-Pro(Act)+ICL}} &
\multicolumn{2}{c}{\textbf{Matrix OT+ICL}} &
\multicolumn{2}{c}{\textbf{OT-PCA(Act)+ICL}} &
\multicolumn{2}{c}{\textbf{SF Projector+ICL}} &
\multicolumn{2}{c}{\textbf{OT-Embed(Act)+ICL}} 
\\

\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}

\textbf{Metric}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}with norm\end{tabular}
& \begin{tabular}[c]{@{}c@{}}w/o norm\end{tabular}
\\
\midrule

%----------------------------------------------------------------
% PEARSON
%----------------------------------------------------------------
\textbf{Pearson} 
& 0.509    % Ran-Pro(Act)+ICL (with norm) => icrl_act_Ran-Pro_icl
& --       % Ran-Pro(Act)+ICL (w/o norm) => (not available)
& 0.509    % Matrix OT+ICL (with norm) => matrix_ot_Ran-Pro_icl
& --       % Matrix OT+ICL (w/o norm)
& \textbf{0.549} % OT-PCA(Act)+ICL (with norm) => pca_ot_act_Ran-Pro_icl
& \underline{0.538} % OT-PCA(Act)+ICL (w/o norm) => pca_ot_act_Ran-Pro_icl_w_o_norm
& 0.515    % SF Projector+ICL (with norm) => sf_projector_Ran-Pro_icl
& --       % SF Projector+ICL (w/o norm)
& 0.534    % OT-Embed(Act)+ICL (with norm) => embed_ot_act_Ran-Pro_icl
& 0.536    % OT-Embed(Act)+ICL (w/o norm) => embed_ot_act_Ran-Pro_icl_w_o_norm
\\

%----------------------------------------------------------------
% SPEARMAN
%----------------------------------------------------------------
\textbf{Spearman} 
& 0.518    % Ran-Pro(Act)+ICL (with norm) => icrl_act_Ran-Pro_icl
& --       % w/o norm
& 0.518    % Matrix OT+ICL (with norm) => matrix_ot_Ran-Pro_icl
& --       % w/o norm
& 0.564    % OT-PCA(Act)+ICL (with norm) => pca_ot_act_Ran-Pro_icl
& \textbf{0.568} % OT-PCA(Act)+ICL (w/o norm) => pca_ot_act_Ran-Pro_icl_w_o_norm
& 0.548    % SF Projector+ICL (with norm) => sf_projector_Ran-Pro_icl
& --       % w/o norm
& 0.551    % OT-Embed(Act)+ICL (with norm) => embed_ot_act_Ran-Pro_icl
& 0.555    % OT-Embed(Act)+ICL (w/o norm) => embed_ot_act_Ran-Pro_icl_w_o_norm
\\

%----------------------------------------------------------------
% RMSE
%----------------------------------------------------------------
\textbf{RMSE} 
& 1.139    % Ran-Pro(Act)+ICL => icrl_act_Ran-Pro_icl
& --       
& 1.139    % Matrix OT+ICL => matrix_ot_Ran-Pro_icl
& --       
& 1.097    % OT-PCA(Act)+ICL => pca_ot_act_Ran-Pro_icl
& 1.107    % pca_ot_act_Ran-Pro_icl_w_o_norm
& 1.187    % sf_projector_Ran-Pro_icl
& --       
& \textbf{1.081} % embed_ot_act_Ran-Pro_icl
& \underline{1.094} % embed_ot_act_Ran-Pro_icl_w_o_norm
\\

\bottomrule
\end{tabular}
}
\end{table*}


==> Tables/sf.tex <==
\begin{table}[!ht]
\centering
\caption{Comparison of Two Self-Supervised Learning Objectives}
\label{tab:self_supervised_learning}
\small
\renewcommand{\arraystretch}{1.2} % 增加行间距
\setlength{\tabcolsep}{6pt} % 调整列间距
\begin{tabular}{p{4cm}p{5cm}p{5cm}}
\toprule
\textbf{Aspect}                      & \textbf{Objective 1: Text Embedding}    & \textbf{Objective 2: Last Logits} \\ 
\midrule
\textbf{Learning Task}               & Self-supervised learning to learn meaningful text embeddings for Embeddings. & Self-supervised learning focusing on summarizing the input sequence through the last logits. \\ 
\textbf{Experiment Details}          & 
sf\_projector\_Ran-Pro \newline 
sf\_projector\_Ran-Pro\_w\_o\_norm & 
sf\_projector\_match\_logits\_Ran-Pro \newline
sf\_projector\_match\_logits\_Ran-Pro\_icl \\ 
\textbf{Metrics (Best Results)}      & 
Pearson Mean: 0.171 \newline 
RMSE Mean: 1.644 \newline 
Spearman Mean: 0.150 & 
Pearson Mean: 0.520 \newline 
RMSE Mean: 1.020 \newline 
Spearman Mean: 0.520 \\ 
\bottomrule
\end{tabular}
\end{table}


==> Tables/v2.tex <==

\begin{table*}[!ht]
\centering
\small
\caption{
Performance comparison on three metrics (\textit{Per\_cor}, \textit{Ser\_cor}, and \textit{Rmse}) on protein - v2. 
\textbf{Bold} = performance better than \textit{ICL}.
}

\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Metric} & \textbf{ICL} & \textbf{PCA+ICL} & \textbf{OT-PCA+ICL} & \textbf{OT-Embed+ICL} & \textbf{Ran-Pro+ICL} & \textbf{Ran-Noi+ICL} \\ 
\midrule
\textbf{Pearson} & 0.130 & \textit{OOM} & 0.194 & 0.177 & 0.217 & 0.111 \\ 
\textbf{Spearman} & 0.133 & \textit{OOM} & 0.184 & 0.172 & 0.192 & 0.111 \\ 
\textbf{RMSE} & 0.735 & \textit{OOM} & 0.719 & 0.720 & 0.738 & 0.780 \\ 
\bottomrule
\end{tabular}%
}
\end{table*}

==> Tables/zero_shot.tex <==
\begin{table}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\caption{
    Summary of Zero-Shot Experimental Results on Different Methods. 
    \textbf{Bold} = best value (highest for Pearson/Spearman, lowest for RMSE); \underline{Underline} = second-best.
}
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Pearson} & \textbf{Spearman} & \textbf{RMSE} \\ 
\midrule
ICL            & \textbf{0.448 ± 1.2e-3} & \underline{0.484 ± 4.3e-4} & 3.492 ± 5.3e-4 \\ 
PCA            & 0.015 ± 7.1e-4          & 0.005 ± 1.1e-3             & \underline{2.805 ± 7.5e-3} \\ 
PCA+ICL        & \underline{0.445 ± 2.0e-3} & 0.449 ± 4.7e-3             & 3.153 ± 6.0e-3 \\ 
OT-PCA         & 0.136 ± 2.0e-1          & 0.133 ± 1.3e-1             & \textbf{1.652 ± 2.6e-1} \\ 
OT-PCA+ICL     & 0.431 ± 3.0e-3          & \textbf{0.504 ± 7.6e-4}    & 3.605 ± 8.2e-3 \\ 
\bottomrule
\end{tabular}
\end{table}
